An improved effective-one-body model of spinning, nonprecessing binary black holes for the era of gravitational-wave astrophysics with advanced detectors

We improve the accuracy of the effective-one-body (EOB) waveforms that were employed during the first observing run of Advanced LIGO for binaries of spinning, nonprecessing black holes by calibrating them to a set of 141 numerical-relativity (NR) waveforms. The NR simulations expand the domain of calibration towards larger mass ratios and spins, as compared to the previous EOBNR model. Merger-ringdown waveforms computed in black-hole perturbation theory for Kerr spins close to extremal provide additional inputs to the calibration. For the inspiral-plunge phase, we use a Markov-chain Monte Carlo algorithm to efficiently explore the calibration space. For the merger-ringdown phase, we fit the NR signals with phenomenological formulae. After extrapolation of the calibrated model to arbitrary mass ratios and spins, the (dominant-mode) EOBNR waveforms have faithfulness --- at design Advanced-LIGO sensitivity --- above $99\%$ against all the NR waveforms, including 16 additional waveforms used for validation, when maximizing only on initial phase and time. This implies a negligible loss in event rate due to modeling for these binary configurations. We find that future NR simulations at mass ratios $\gtrsim 4$ and double spin $\gtrsim 0.8$ will be crucial to resolve discrepancies between different ways of extrapolating waveform models. We also find that some of the NR simulations that already exist in such region of parameter space are too short to constrain the low-frequency portion of the models. Finally, we build a reduced-order version of the EOBNR model to speed up waveform generation by orders of magnitude, thus enabling intensive data-analysis applications during the upcoming observation runs of Advanced LIGO.

==> tables/allnrsims.tex <==
%\begin{tabular}{lllllll}
ID & $q$ & $\chi_1$ & $\chi_2$ & $e$ & $M\omega$ & $N_\mathrm{orb}$\\
\hline
\endfirsthead
ID & $q$ & $\chi_1$ & $\chi_2$ & $e$ & $M\omega$ & $N_\mathrm{orb}$\\
\hline
\endhead
SXS:BBH:0004 & $1.0$ & $-0.50$ & $+0.00$ & $3.7\times 10^{-4}$ & $0.01151$ & $30.2$ \\
SXS:BBH:0005 & $1.0$ & $+0.50$ & $+0.00$ & $2.5\times 10^{-4}$ & $0.01227$ & $30.2$ \\
SXS:BBH:0007 & $1.5$ & $+0.00$ & $+0.00$ & $4.2\times 10^{-4}$ & $0.01229$ & $29.1$ \\
SXS:BBH:0013 & $1.5$ & $+0.50$ & $+0.00$ & $1.4\times 10^{-4}$ & $0.01444$ & $23.8$ \\
SXS:BBH:0016 & $1.5$ & $-0.50$ & $+0.00$ & $4.2\times 10^{-4}$ & $0.01149$ & $30.7$ \\
SXS:BBH:0019 & $1.5$ & $-0.50$ & $+0.50$ & $7.6\times 10^{-5}$ & $0.01460$ & $20.4$ \\
SXS:BBH:0025 & $1.5$ & $+0.50$ & $-0.50$ & $7.6\times 10^{-5}$ & $0.01456$ & $22.4$ \\
SXS:BBH:0030 & $3.0$ & $+0.00$ & $+0.00$ & $2.0\times 10^{-3}$ & $0.01775$ & $18.2$ \\
SXS:BBH:0036 & $3.0$ & $-0.50$ & $+0.00$ & $5.1\times 10^{-4}$ & $0.01226$ & $31.7$ \\
SXS:BBH:0045 & $3.0$ & $+0.50$ & $-0.50$ & $6.4\times 10^{-4}$ & $0.01748$ & $21.0$ \\
SXS:BBH:0046 & $3.0$ & $-0.50$ & $-0.50$ & $2.6\times 10^{-4}$ & $0.01771$ & $14.4$ \\
SXS:BBH:0047 & $3.0$ & $+0.50$ & $+0.50$ & $4.7\times 10^{-4}$ & $0.01743$ & $22.7$ \\
SXS:BBH:0056 & $5.0$ & $+0.00$ & $+0.00$ & $4.9\times 10^{-4}$ & $0.01589$ & $28.8$ \\
SXS:BBH:0060 & $5.0$ & $-0.50$ & $+0.00$ & $3.4\times 10^{-3}$ & $0.01608$ & $23.2$ \\
SXS:BBH:0061 & $5.0$ & $+0.50$ & $+0.00$ & $4.2\times 10^{-3}$ & $0.01578$ & $34.5$ \\
SXS:BBH:0063 & $8.0$ & $+0.00$ & $+0.00$ & $2.8\times 10^{-4}$ & $0.01938$ & $25.8$ \\
SXS:BBH:0064 & $8.0$ & $-0.50$ & $+0.00$ & $4.9\times 10^{-4}$ & $0.01968$ & $19.2$ \\
SXS:BBH:0065 & $8.0$ & $+0.50$ & $+0.00$ & $3.7\times 10^{-3}$ & $0.01887$ & $34.0$ \\
SXS:BBH:0148 & $1.0$ & $-0.44$ & $-0.44$ & $2.0\times 10^{-5}$ & $0.01634$ & $15.5$ \\
SXS:BBH:0149 & $1.0$ & $-0.20$ & $-0.20$ & $1.8\times 10^{-4}$ & $0.01614$ & $17.1$ \\
SXS:BBH:0150 & $1.0$ & $+0.20$ & $+0.20$ & $2.9\times 10^{-4}$ & $0.01591$ & $19.8$ \\
SXS:BBH:0151 & $1.0$ & $-0.60$ & $-0.60$ & $2.5\times 10^{-4}$ & $0.01575$ & $14.5$ \\
SXS:BBH:0152 & $1.0$ & $+0.60$ & $+0.60$ & $4.3\times 10^{-4}$ & $0.01553$ & $22.6$ \\
SXS:BBH:0153 & $1.0$ & $+0.85$ & $+0.85$ & $8.3\times 10^{-4}$ & $0.01539$ & $24.5$ \\
SXS:BBH:0154 & $1.0$ & $-0.80$ & $-0.80$ & $3.3\times 10^{-4}$ & $0.01605$ & $13.2$ \\
SXS:BBH:0155 & $1.0$ & $+0.80$ & $+0.80$ & $4.7\times 10^{-4}$ & $0.01543$ & $24.1$ \\
SXS:BBH:0156 & $1.0$ & $-0.95$ & $-0.95$ & $5.4\times 10^{-4}$ & $0.01643$ & $12.4$ \\
SXS:BBH:0157 & $1.0$ & $+0.95$ & $+0.95$ & $1.4\times 10^{-4}$ & $0.01535$ & $25.2$ \\
SXS:BBH:0158 & $1.0$ & $+0.97$ & $+0.97$ & $7.9\times 10^{-4}$ & $0.01565$ & $25.3$ \\
SXS:BBH:0159 & $1.0$ & $-0.90$ & $-0.90$ & $5.6\times 10^{-4}$ & $0.01588$ & $12.7$ \\
SXS:BBH:0160 & $1.0$ & $+0.90$ & $+0.90$ & $4.2\times 10^{-4}$ & $0.01538$ & $24.8$ \\
SXS:BBH:0166 & $6.0$ & $+0.00$ & $+0.00$ & $4.4\times 10^{-5}$ & $0.01940$ & $21.6$ \\
SXS:BBH:0167 & $4.0$ & $+0.00$ & $+0.00$ & $9.9\times 10^{-5}$ & $0.02054$ & $15.6$ \\
SXS:BBH:0169 & $2.0$ & $+0.00$ & $+0.00$ & $1.2\times 10^{-4}$ & $0.01799$ & $15.7$ \\
SXS:BBH:0170 & $1.0$ & $+0.44$ & $+0.44$ & $1.3\times 10^{-4}$ & $0.00842$ & $15.5$ \\
SXS:BBH:0172 & $1.0$ & $+0.98$ & $+0.98$ & $7.8\times 10^{-4}$ & $0.01540$ & $25.4$ \\
SXS:BBH:0174 & $3.0$ & $+0.50$ & $+0.00$ & $2.9\times 10^{-4}$ & $0.01337$ & $35.5$ \\
SXS:BBH:0177 & $1.0$ & $+0.99$ & $+0.99$ & $1.3\times 10^{-3}$ & $0.01543$ & $25.4$ \\
SXS:BBH:0178 & $1.0$ & $+0.99$ & $+0.99$ & $8.6\times 10^{-4}$ & $0.01570$ & $25.4$ \\
SXS:BBH:0180 & $1.0$ & $+0.00$ & $+0.00$ & $5.1\times 10^{-5}$ & $0.01227$ & $28.2$ \\
SXS:BBH:0202 & $7.0$ & $+0.60$ & $+0.00$ & $9.0\times 10^{-5}$ & $0.01324$ & $62.1$ \\
SXS:BBH:0203 & $7.0$ & $+0.40$ & $+0.00$ & $1.4\times 10^{-5}$ & $0.01322$ & $58.5$ \\
SXS:BBH:0204 & $7.0$ & $+0.40$ & $+0.00$ & $1.7\times 10^{-4}$ & $0.01044$ & $88.4$ \\
SXS:BBH:0205 & $7.0$ & $-0.40$ & $+0.00$ & $7.0\times 10^{-5}$ & $0.01325$ & $44.9$ \\
SXS:BBH:0206 & $7.0$ & $-0.40$ & $+0.00$ & $1.6\times 10^{-4}$ & $0.01037$ & $73.2$ \\
SXS:BBH:0207 & $7.0$ & $-0.60$ & $+0.00$ & $1.7\times 10^{-4}$ & $0.01423$ & $36.1$ \\
SXS:BBH:0306 & $1.3$ & $+0.96$ & $-0.90$ & $1.5\times 10^{-3}$ & $0.02098$ & $12.6$ \\
SXS:BBH:0290 & $3.0$ & $+0.60$ & $+0.40$ & $9.0\times 10^{-5}$ & $0.01758$ & $24.2$ \\
SXS:BBH:0291 & $3.0$ & $+0.60$ & $+0.60$ & $5.0\times 10^{-5}$ & $0.01764$ & $24.5$ \\
SXS:BBH:0289 & $3.0$ & $+0.60$ & $+0.00$ & $2.3\times 10^{-4}$ & $0.01711$ & $23.8$ \\
SXS:BBH:0285 & $3.0$ & $+0.40$ & $+0.60$ & $1.6\times 10^{-4}$ & $0.01732$ & $23.8$ \\
SXS:BBH:0261 & $3.0$ & $-0.73$ & $+0.85$ & $1.0\times 10^{-4}$ & $0.01490$ & $21.5$ \\
SXS:BBH:0293 & $3.0$ & $+0.85$ & $+0.85$ & $9.0\times 10^{-5}$ & $0.01813$ & $25.6$ \\
SXS:BBH:0280 & $3.0$ & $+0.27$ & $+0.85$ & $9.7\times 10^{-5}$ & $0.01707$ & $23.6$ \\
SXS:BBH:0257 & $2.0$ & $+0.85$ & $+0.85$ & $1.1\times 10^{-4}$ & $0.01633$ & $24.8$ \\
SXS:BBH:0279 & $3.0$ & $+0.23$ & $-0.85$ & $6.0\times 10^{-5}$ & $0.01629$ & $22.6$ \\
SXS:BBH:0274 & $3.0$ & $-0.23$ & $+0.85$ & $1.6\times 10^{-4}$ & $0.01603$ & $22.4$ \\
SXS:BBH:0258 & $2.0$ & $+0.87$ & $-0.85$ & $1.8\times 10^{-4}$ & $0.01612$ & $22.8$ \\
SXS:BBH:0248 & $2.0$ & $+0.13$ & $+0.85$ & $7.0\times 10^{-5}$ & $0.01552$ & $23.2$ \\
SXS:BBH:0232 & $1.0$ & $+0.90$ & $+0.50$ & $2.8\times 10^{-4}$ & $0.01558$ & $23.9$ \\
SXS:BBH:0229 & $1.0$ & $+0.65$ & $+0.25$ & $3.1\times 10^{-4}$ & $0.01488$ & $23.1$ \\
SXS:BBH:0231 & $1.0$ & $+0.90$ & $+0.00$ & $1.0\times 10^{-4}$ & $0.01487$ & $23.1$ \\
SXS:BBH:0239 & $2.0$ & $-0.37$ & $+0.85$ & $9.1\times 10^{-5}$ & $0.01478$ & $22.2$ \\
SXS:BBH:0252 & $2.0$ & $+0.37$ & $-0.85$ & $3.8\times 10^{-4}$ & $0.01488$ & $22.5$ \\
SXS:BBH:0219 & $1.0$ & $-0.50$ & $+0.90$ & $3.3\times 10^{-4}$ & $0.01484$ & $22.4$ \\
SXS:BBH:0211 & $1.0$ & $-0.90$ & $+0.90$ & $2.6\times 10^{-4}$ & $0.01411$ & $22.3$ \\
SXS:BBH:0233 & $2.0$ & $-0.87$ & $+0.85$ & $6.0\times 10^{-5}$ & $0.01423$ & $22.0$ \\
SXS:BBH:0243 & $2.0$ & $-0.13$ & $-0.85$ & $1.8\times 10^{-4}$ & $0.01378$ & $23.3$ \\
SXS:BBH:0214 & $1.0$ & $-0.62$ & $-0.25$ & $1.9\times 10^{-4}$ & $0.01264$ & $24.4$ \\
SXS:BBH:0209 & $1.0$ & $-0.90$ & $-0.50$ & $1.7\times 10^{-4}$ & $0.01137$ & $27.0$ \\
SXS:BBH:0226 & $1.0$ & $+0.50$ & $-0.90$ & $2.4\times 10^{-4}$ & $0.01340$ & $22.9$ \\
SXS:BBH:0286 & $3.0$ & $+0.50$ & $+0.50$ & $8.0\times 10^{-5}$ & $0.01693$ & $24.1$ \\
SXS:BBH:0253 & $2.0$ & $+0.50$ & $+0.50$ & $6.7\times 10^{-5}$ & $0.01397$ & $28.8$ \\
SXS:BBH:0267 & $3.0$ & $-0.50$ & $-0.50$ & $5.6\times 10^{-5}$ & $0.01410$ & $23.4$ \\
SXS:BBH:0218 & $1.0$ & $-0.50$ & $+0.50$ & $7.8\times 10^{-5}$ & $0.01217$ & $29.1$ \\
SXS:BBH:0238 & $2.0$ & $-0.50$ & $-0.50$ & $6.9\times 10^{-5}$ & $0.01126$ & $32.0$ \\
SXS:BBH:0288 & $3.0$ & $+0.60$ & $-0.40$ & $1.9\times 10^{-4}$ & $0.01729$ & $23.5$ \\
SXS:BBH:0287 & $3.0$ & $+0.60$ & $-0.60$ & $7.0\times 10^{-5}$ & $0.01684$ & $23.5$ \\
SXS:BBH:0283 & $3.0$ & $+0.30$ & $+0.30$ & $7.6\times 10^{-5}$ & $0.01646$ & $23.5$ \\
SXS:BBH:0282 & $3.0$ & $+0.30$ & $+0.00$ & $7.5\times 10^{-5}$ & $0.01629$ & $23.3$ \\
SXS:BBH:0281 & $3.0$ & $+0.30$ & $-0.30$ & $6.7\times 10^{-5}$ & $0.01618$ & $23.2$ \\
SXS:BBH:0277 & $3.0$ & $+0.00$ & $+0.30$ & $7.0\times 10^{-5}$ & $0.01595$ & $22.9$ \\
SXS:BBH:0284 & $3.0$ & $+0.40$ & $-0.60$ & $1.5\times 10^{-4}$ & $0.01656$ & $22.8$ \\
SXS:BBH:0278 & $3.0$ & $+0.00$ & $+0.60$ & $2.1\times 10^{-4}$ & $0.01623$ & $22.8$ \\
SXS:BBH:0256 & $2.0$ & $+0.60$ & $+0.60$ & $1.0\times 10^1$ & $0.01598$ & $23.9$ \\
SXS:BBH:0230 & $1.0$ & $+0.80$ & $+0.80$ & $1.3\times 10^{-4}$ & $0.01542$ & $24.2$ \\
SXS:BBH:0255 & $2.0$ & $+0.60$ & $+0.00$ & $4.0\times 10^{-5}$ & $0.01580$ & $23.3$ \\
SXS:BBH:0276 & $3.0$ & $+0.00$ & $-0.30$ & $6.7\times 10^{-5}$ & $0.01559$ & $23.0$ \\
SXS:BBH:0251 & $2.0$ & $+0.30$ & $+0.30$ & $7.5\times 10^{-5}$ & $0.01514$ & $23.5$ \\
SXS:BBH:0250 & $2.0$ & $+0.30$ & $+0.00$ & $7.5\times 10^{-5}$ & $0.01503$ & $23.2$ \\
SXS:BBH:0271 & $3.0$ & $-0.30$ & $+0.00$ & $6.3\times 10^{-5}$ & $0.01508$ & $22.5$ \\
SXS:BBH:0249 & $2.0$ & $+0.30$ & $-0.30$ & $7.2\times 10^{-5}$ & $0.01478$ & $23.2$ \\
SXS:BBH:0275 & $3.0$ & $+0.00$ & $-0.60$ & $1.2\times 10^{-4}$ & $0.01569$ & $22.6$ \\
SXS:BBH:0254 & $2.0$ & $+0.60$ & $-0.60$ & $6.0\times 10^{-5}$ & $0.01541$ & $22.9$ \\
SXS:BBH:0269 & $3.0$ & $-0.40$ & $+0.60$ & $1.2\times 10^{-4}$ & $0.01563$ & $22.3$ \\
SXS:BBH:0225 & $1.0$ & $+0.40$ & $+0.80$ & $3.5\times 10^{-4}$ & $0.01536$ & $23.5$ \\
SXS:BBH:0270 & $3.0$ & $-0.30$ & $-0.30$ & $6.2\times 10^{-5}$ & $0.01482$ & $22.8$ \\
SXS:BBH:0245 & $2.0$ & $+0.00$ & $-0.30$ & $6.8\times 10^{-5}$ & $0.01441$ & $23.0$ \\
SXS:BBH:0242 & $2.0$ & $-0.30$ & $+0.30$ & $6.7\times 10^{-5}$ & $0.01417$ & $23.1$ \\
SXS:BBH:0223 & $1.0$ & $+0.30$ & $+0.00$ & $6.7\times 10^{-5}$ & $0.01402$ & $23.3$ \\
SXS:BBH:0241 & $2.0$ & $-0.30$ & $+0.00$ & $6.6\times 10^{-5}$ & $0.01394$ & $23.1$ \\
SXS:BBH:0240 & $2.0$ & $-0.30$ & $-0.30$ & $6.4\times 10^{-5}$ & $0.01359$ & $23.5$ \\
SXS:BBH:0222 & $1.0$ & $-0.30$ & $+0.00$ & $7.4\times 10^{-5}$ & $0.01324$ & $23.6$ \\
SXS:BBH:0228 & $1.0$ & $+0.60$ & $+0.60$ & $3.2\times 10^{-4}$ & $0.01543$ & $23.5$ \\
SXS:BBH:0247 & $2.0$ & $+0.00$ & $+0.60$ & $1.0\times 10^{-4}$ & $0.01530$ & $22.6$ \\
SXS:BBH:0263 & $3.0$ & $-0.60$ & $+0.60$ & $1.9\times 10^{-4}$ & $0.01526$ & $22.0$ \\
SXS:BBH:0266 & $3.0$ & $-0.60$ & $+0.40$ & $1.8\times 10^{-4}$ & $0.01488$ & $22.0$ \\
SXS:BBH:0227 & $1.0$ & $+0.60$ & $+0.00$ & $3.1\times 10^{-4}$ & $0.01452$ & $23.1$ \\
SXS:BBH:0221 & $1.0$ & $-0.40$ & $+0.80$ & $2.7\times 10^{-4}$ & $0.01440$ & $22.7$ \\
SXS:BBH:0237 & $2.0$ & $-0.60$ & $+0.60$ & $6.1\times 10^{-5}$ & $0.01433$ & $22.6$ \\
SXS:BBH:0244 & $2.0$ & $+0.00$ & $-0.60$ & $7.5\times 10^{-5}$ & $0.01422$ & $23.2$ \\
SXS:BBH:0217 & $1.0$ & $-0.60$ & $+0.60$ & $1.5\times 10^{-4}$ & $0.01421$ & $22.7$ \\
SXS:BBH:0215 & $1.0$ & $-0.60$ & $-0.60$ & $1.8\times 10^{-4}$ & $0.01189$ & $25.8$ \\
SXS:BBH:0262 & $3.0$ & $-0.60$ & $+0.00$ & $2.0\times 10^{-4}$ & $0.01473$ & $22.5$ \\
SXS:BBH:0213 & $1.0$ & $-0.80$ & $+0.80$ & $1.4\times 10^{-4}$ & $0.01435$ & $22.3$ \\
SXS:BBH:0265 & $3.0$ & $-0.60$ & $-0.40$ & $9.0\times 10^{-5}$ & $0.01422$ & $23.4$ \\
SXS:BBH:0264 & $3.0$ & $-0.60$ & $-0.60$ & $2.8\times 10^{-4}$ & $0.01410$ & $23.4$ \\
SXS:BBH:0224 & $1.0$ & $+0.40$ & $-0.80$ & $2.5\times 10^{-4}$ & $0.01361$ & $22.9$ \\
SXS:BBH:0236 & $2.0$ & $-0.60$ & $+0.00$ & $1.2\times 10^{-4}$ & $0.01361$ & $23.4$ \\
SXS:BBH:0216 & $1.0$ & $-0.60$ & $+0.00$ & $2.6\times 10^{-4}$ & $0.01300$ & $23.6$ \\
SXS:BBH:0235 & $2.0$ & $-0.60$ & $-0.60$ & $1.0\times 10^1$ & $0.01274$ & $25.1$ \\
SXS:BBH:0220 & $1.0$ & $-0.40$ & $-0.80$ & $1.0\times 10^{-4}$ & $0.01195$ & $25.7$ \\
SXS:BBH:0212 & $1.0$ & $-0.80$ & $-0.80$ & $2.4\times 10^{-4}$ & $0.01087$ & $28.6$ \\
SXS:BBH:0303 & $10.0$ & $+0.00$ & $+0.00$ & $5.1\times 10^{-5}$ & $0.02395$ & $19.3$ \\
SXS:BBH:0300 & $8.5$ & $+0.00$ & $+0.00$ & $5.7\times 10^{-5}$ & $0.02311$ & $18.7$ \\
SXS:BBH:0299 & $7.5$ & $+0.00$ & $+0.00$ & $5.9\times 10^{-5}$ & $0.02152$ & $20.1$ \\
SXS:BBH:0298 & $7.0$ & $+0.00$ & $+0.00$ & $6.1\times 10^{-5}$ & $0.02130$ & $19.7$ \\
SXS:BBH:0297 & $6.5$ & $+0.00$ & $+0.00$ & $6.4\times 10^{-5}$ & $0.02082$ & $19.7$ \\
SXS:BBH:0296 & $5.5$ & $+0.00$ & $+0.00$ & $5.2\times 10^{-5}$ & $0.01668$ & $27.9$ \\
SXS:BBH:0295 & $4.5$ & $+0.00$ & $+0.00$ & $5.2\times 10^{-5}$ & $0.01577$ & $27.8$ \\
SXS:BBH:0259 & $2.5$ & $+0.00$ & $+0.00$ & $5.9\times 10^{-5}$ & $0.01346$ & $28.6$ \\
SXS:BBH:0292 & $3.0$ & $+0.73$ & $-0.85$ & $1.8\times 10^{-4}$ & $0.01749$ & $23.9$ \\
SXS:BBH:0268 & $3.0$ & $-0.40$ & $-0.60$ & $1.7\times 10^{-4}$ & $0.01473$ & $22.9$ \\
SXS:BBH:0234 & $2.0$ & $-0.85$ & $-0.85$ & $1.4\times 10^{-4}$ & $0.01147$ & $27.8$ \\
SXS:BBH:0273 & $3.0$ & $-0.27$ & $-0.85$ & $2.0\times 10^{-4}$ & $0.01487$ & $22.9$ \\
SXS:BBH:0210 & $1.0$ & $-0.90$ & $+0.00$ & $1.8\times 10^{-4}$ & $0.01248$ & $24.3$ \\
SXS:BBH:0260 & $3.0$ & $-0.85$ & $-0.85$ & $3.5\times 10^{-4}$ & $0.01285$ & $25.8$ \\
SXS:BBH:0302 & $9.5$ & $+0.00$ & $+0.00$ & $6.0\times 10^{-5}$ & $0.02366$ & $19.1$ \\
SXS:BBH:0301 & $9.0$ & $+0.00$ & $+0.00$ & $5.5\times 10^{-5}$ & $0.02338$ & $18.9$ \\
SXS:BBH:0272 & $3.0$ & $-0.30$ & $+0.30$ & $6.4\times 10^{-5}$ & $0.01521$ & $22.7$ \\
SXS:BBH:0246 & $2.0$ & $+0.00$ & $+0.30$ & $7.2\times 10^{-5}$ & $0.01514$ & $22.9$ \\
%\end{tabular}


==> tables/nrsims.tex <==
\begin{tabular}{lllllll}
Id & $q$ & $\chi_1$ & $\chi_2$ & $e$ & $M\omega$ & $N_\mathrm{orb}$\\
\hline
SXS:BBH:0610 & $1.2$ & $-0.50$ & $-0.50$ & $7.4\times 10^{-5}$ & $0.01872$ & $12.1$ \\
SXS:BBH:0611 & $1.4$ & $-0.50$ & $+0.50$ & $6.0\times 10^{-4}$ & $0.02033$ & $12.5$ \\
SXS:BBH:0612 & $1.6$ & $+0.50$ & $-0.50$ & $3.7\times 10^{-4}$ & $0.02156$ & $12.8$ \\
SXS:BBH:0613 & $1.8$ & $+0.50$ & $+0.50$ & $1.8\times 10^{-4}$ & $0.02383$ & $13.1$ \\
SXS:BBH:0614 & $2.0$ & $+0.75$ & $-0.50$ & $6.7\times 10^{-4}$ & $0.02355$ & $13.1$ \\
SXS:BBH:0615 & $2.0$ & $+0.75$ & $+0.00$ & $7.0\times 10^{-4}$ & $0.02401$ & $13.3$ \\
SXS:BBH:0616 & $2.0$ & $+0.75$ & $+0.50$ & $8.0\times 10^{-4}$ & $0.02475$ & $13.3$ \\
SXS:BBH:0617 & $2.0$ & $+0.50$ & $+0.75$ & $7.8\times 10^{-4}$ & $0.02342$ & $13.1$ \\
SXS:BBH:0618 & $2.0$ & $+0.80$ & $+0.80$ & $5.9\times 10^{-4}$ & $0.02578$ & $13.4$ \\
SXS:BBH:0619 & $2.0$ & $+0.90$ & $+0.90$ & $2.9\times 10^{-4}$ & $0.02520$ & $13.5$ \\
SXS:BBH:0620 & $5.0$ & $-0.80$ & $+0.00$ & $1.7\times 10^{-4}$ & $0.02551$ & $8.1$ \\
SXS:BBH:0621 & $7.0$ & $-0.80$ & $+0.00$ & $4.8\times 10^{-4}$ & $0.02828$ & $7.2$ \\
SXS:BBH:0622 & $8.0$ & $-0.90$ & $+0.00$ & $1.1\times 10^{-3}$ & $0.01559$ & $28.0$ \\
\hline
ET:AEI:0001 & $5.0$ & $+0.80$ & $+0.00$ & $9.2\times 10^{-4}$ & $0.03077$ & $10.5$ \\
ET:AEI:0002 & $7.0$ & $+0.80$ & $+0.00$ & $6.1\times 10^{-4}$ & $0.03503$ & $10.4$ \\
ET:AEI:0003 & $8.0$ & $+0.85$ & $+0.85$ & $1.2\times 10^{-2}$ & $0.04099$ & $7.4$ \\
\end{tabular}

